Near-linear Size Hypergraph Cut Sparsifiers

Cuts in graphs are a fundamental object of study, and play a central role in the study of graph algorithms. The problem of sparsifying a graph while approximately preserving its cut structure has been extensively studied and has many applications. In a seminal work, Bencz\'ur and Karger (1996) showed that given any $n$-vertex undirected weighted graph $G$ and a parameter $\varepsilon \in (0,1)$, there is a near-linear time algorithm that outputs a weighted subgraph $G'$ of $G$ of size $\tilde{O}(n/\varepsilon^2)$ such that the weight of every cut in $G$ is preserved to within a $(1 \pm \varepsilon)$-factor in $G'$. The graph $G'$ is referred to as a {\em $(1 \pm \varepsilon)$-approximate cut sparsifier} of $G$. A natural question is if such cut-preserving sparsifiers also exist for hypergraphs. Kogan and Krauthgamer (2015) initiated a study of this question and showed that given any weighted hypergraph $H$ where the cardinality of each hyperedge is bounded by $r$, there is a polynomial-time algorithm to find a $(1 \pm \varepsilon)$-approximate cut sparsifier of $H$ of size $\tilde{O}(\frac{nr}{\varepsilon^2})$. Since $r$ can be as large as $n$, in general, this gives a hypergraph cut sparsifier of size $\tilde{O}(n^2/\varepsilon^2)$, which is a factor $n$ larger than the Bencz\'ur-Karger bound for graphs. It has been an open question whether or not Bencz\'ur-Karger bound is achievable on hypergraphs. In this work, we resolve this question in the affirmative by giving a new polynomial-time algorithm for creating hypergraph sparsifiers of size $\tilde{O}(n/\varepsilon^2)$.

==> balance_backup.tex <==
\section{Find a $\gamma$-balanced Assignment} \label{sec:balance}

In this section, we prove Theorem~\ref{thm:balance}, which shows that given an unweighted hypergraph $H=(V,E)$ with $n$ vertices and $m$ hyperedges, and for any $\gamma \ge 2$, we can find a $\gamma$-balanced assignment in $m^{O(\log_{\gamma} m)}$ time. To simplify the exposition, we will show how to find a $\gamma^2$-balanced assigment instead in $m^{O(\log_{\gamma} m)}$ time, which immediately implies that we can also find a $\gamma$-balanced assigment in $m^{O(\log_{\sqrt{\gamma}} m)} = m^{O(\log_{\gamma} m)}$ time.

We find a $\gamma^2$-balanced assignment using an iterative algorithm. We start with the uniform weight assignment. In each step, say $e$ is an unbalanced hyperedge (i.e. $e$ violates condition (2) of Definition \ref{def:balance}) where $f_1$ and $f_2$ are the two edges in $F_e$ that ``witness'' $e$ being unbalanced, i.e. $f_1$ has positive weight and $k_{f_1} > \gamma k_{f_2}$. We move weight from $f_1$ to $f_2$. Imformally (we will prove later), the strength of $f_1$ can only decrease and the strength of $f_2$ can only increase as a result of this weight transition. There are two possible events that may happen if we keep moving weight from $f_1$ to $f_2$: the strength of $f_1$ becomes closer to $f_2$ and finally their strengths are within a factor of $\gamma$; or even if we move all weight of $f_1$ to $f_2$, $k_{f_1}$ is still larger than $\gamma k_{f_2}$. In both cases, $f_1$ and $f_2$ are no longer a pair of ``witnesses'' to $e$ being unbalanced. We keep doing this until no unbalanced edge remains.

Before we formally describe the algorithm, we first prove a lemma that shows how the strength of edges in a graph change when we change the weight of an edge.

\begin{lemma} \label{lem:change}
    Given a weighted graph $G$ and an edge $e$ in $G$, suppose we increase (resp. decrease) the weight of $e$ by $w$. Then for any edge $e'$ in the graph, the strength of $e'$ does not decrease (resp. increase) and increase (resp. decrease) by at most $w$. Furthermore, if the strength of $e'$ does increase (resp. decrease), the strengh of $e'$ is at least (resp. at most) the strength of $e$ before the change and at most (resp. at least) the stength of $e$ after the change. 
\end{lemma}

\begin{proof}
    For any edge $e'$ in $G$, let $k_{e'}$ be the old strengh and $k'_{e'}$ be the strength of $e'$ after the weight change. We first prove the case when we increase the weight of $e$. For any edge $e'$, let $G[X_{e'}]$ be the induced subgraph of $G$ that contains $e'$ and has minimum cut size $k_{e'}$ before we change the graph. Since we only increase the weight of some edge $e$, the minimum cut size of $G[X_{e'}]$ will not decrease, which means $k_{e'} \le k'_{e'}$. On the other hand, since the weight of $e$ is increased by $w$, the min cut size of any induced subgraph is increased by at most $w$. So $k'_{e'} \le k_{e'}+w$. 

    Now suppose $k'_{e'} > k_{e'}$. Let $G[X'_{e'}]$ be the induced subgraph of $G$ that contains $e'$ and has minimum cut size $k'_{e'}$ after we change the graph. Since $k'_{e'} > k_{e'}$, the minimum cut size of $G[X'_{e'}]$ is less than $k'_{e'}$, which means $e$ is part of every min cut of $G[X'_{e'}]$ before the weight change. This implies that $k'_e$ is at least the minimum cut of $G[X'_{e'}]$, which is $k'_{e'}$. On the other hand, suppose $G[X_e]$ be the induced subgraph of $G$ that contains $e$ and has minimum cut size $k_e$ before we change the graph. Consider the graph $G[X'_{e'} \cup X_{e}]$. Let $C=(S,\bar{S})$ be the minimum cut of this induced subgraph before the weight change, let $c$ be the size of $C$. By definition $c$ is at most $k_{e'}$ since $G[X'_{e'} \cup X_e]$ contains $e'$. If $C$ does not cut through $G[X_e]$, $C$ does not cut through $e$ and it has size $c$ also in $G[X'_{e'}]$. This implies even after the weight change, the minimum cut of $G[X'_{e'}]$ is at most $c$, which means $k'_{e'} \le c \le k_{e'}$ which is a contradiction. So $C$ does cut through $G[X_e]$, which means $c$ is at least the min cut size of $G[X_e]$, and therefore $k_e \le c \le k_{e'}$.

    For the case when we decrease the weight of $e$, we can reverse the role of old graph and new graph, and use the same argument as the proof of the case of increasing the weight of $e$. 
\end{proof}

\subsection{The Algorithm}

Now we describe the algorithm to find a $\gamma^2$-balanced assignment. First we define the initial weights $w^{init}:F\rightarrow \mathbb{R}_{\geq 0}$ as the uniform assignment of one unit of weight to all edges in $F_e$ for each hyperedgee $e$ in $H$. More precisely, for any $f\in F_e$, $w^{init}(f) = \binom{|e|}{2}^{-1}$. These initial weights give us a set of initial edge strengths $k^{init}_f$ of the weighted graph $G^{init} = (V, F, w^{init})$. Define $K_{\min} := \min_{f\in F}k^{init}_f$, and define $K_{\max}$ to be the smallest value larger than $\max_{f\in F}k^{init}_f$ that equals $K_{\min} \cdot \gamma^{\ell}$ for some integer $\ell$. We partition the interval $I=[K_{\min}, K_{\max}]$ into geometrically increasing subintervals $I_1, I_2, \ldots, I_{\ell}$, where $I_j := [K_{\min} \cdot \gamma^{j-1}, K_{\min} \cdot \gamma^j)$. Note that $\ell$ is at most $\log_{\gamma}(\frac{K_{\max}}{K_{\min}})$. Since $\max_{f\in F}k_f^{init}$ is at most the total weight of the edges and $K_{\min}$ is at least $\binom{n}{2}^{-1}$, $\ell$ is at most $\log_{\gamma}(n^2m)$. We fix this partition for the rest of this section.

We use this partition $I_1, I_2, \ldots, I_{\ell}$ to determine how to iteratively modify these weights. Given a real number $x\in I$, we define $\ind(x)$ to be the integer $j$ such that $x\in I_j$. Given a weight function $w^F:F\rightarrow \mathbb{R}_{\geq 0}$ and the corresponding edge strengths $k:F\rightarrow \mathbb{R}_{\geq 0}$, we say that a hyperedge $e\in E$ is \emph{bad} in $G = (V, F, w^F)$ if there exist some $f,f'\in F_e$ such that $w^F(f')>0$ and $\ind(k_f)\leq \ind(k_{f'}) - 2$. That is, $f$ and $f'$ are separated by at least one geometric interval, it is clear that if a hyperedge is not bad, then it is $\gamma^2$-balanced. We note that in general, as we update the weights, $k_f$ and $k_{f'}$ might not be contained in $I$ (so $\ind(k_f)$ might not be defined), but as it will turn out that we will maintain the invariant that all the edge strengths are always contained in $I$. We expand this definition to $\ind(e):=\ind(\max_{f \in F_e^+} k_f)$.

We now invoke the algorithm ${\rm Balance}(w^{init},\ell)$. The algorithm ${\rm Balance}$ takes two parameters $w$ and $i$, which returns a new weight function $w$ such that for each hyperedge $e$ with $\ind(e) \le i$, it is not a bad hyperedge. The algorithm works as follows, if $i \le 2$, then there is nothing to be done, since any hyperedge $e$ with $\ind(e) \le 2$ cannot be bad. If $i>2$, we first run ${\rm Balance}(w,i-1)$ to ensure there is no hyperedge $e$ with $\ind(e) < i$ that is bad. Then if there is any hyperedge $e$ such that $\ind(e) = i$, we balance it by moving the weights from $f_{\max}$ to $f_{\min}$ such that $f_{\max}$ is the maximum strength edge in $F_e^+$ and $f_{\min}$ is the minimum strength edge in $F_e$. After doing this, we run ${\rm Balance}(w,i-1)$ again to make sure there is no bad hyperedge $e$ with $\ind(e) \le i-1$ again.

\vspace{\baselineskip}

\begin{algorithm}[H]\label{alg-balance}
    \caption{A recursive algorithm ${\rm Balance}(w,i)$ that elimates all bad hyperedges with $ind(e) \le i$}
\SetAlgoLined
    \If {$i \le 2$}
    {
        Return $w$\;
    }
    $w={\rm Balance}(w,i-1)$  \;
    \While{there exists some bad edge $e$ such that $ind(e)=i$} {
     Let $f_{\min}:=\arg\min_{f\in F_e}k_f$ and $f_{\max}:=\arg\max_{f\in F_e^+}k_{f}$\;
     Let $k_{\min}$ and $k_{\max}$ to be the strengths of $f_{\min}$ and $f_{\max}$, respectively\; 
     Let $\delta:=\min(w(f_{\max}), (\gamma-1) k_{\min})$\;
     Increase $w(f_{\min})$ by $\delta$ and decrease $w(f_{\max})$ by $\delta$\;
     $w={\rm Balance}(w,i-1)$ \;
 }
 Return $w$\;
\end{algorithm}
\vspace{\baselineskip}

To prove the correctness of the algorithm, we first prove an important invariant that is maintained by the algorithm. 

\begin{claim}\label{cla:interval-contained}
    For any $i$, each time after we change the weights (Line 9), for any edge $f$ such that $k_f$ increases, $\ind(k_f) < i$. Also, no edge $f$ has strength less than $k_{\min}$.
\end{claim}

\begin{proof}
    In each iteration of the while loop, the edge $e$ has $\ind(e) = i$. By definition of $\ind(e)$ and $f_{\max}$, we have $\ind(k_{\max}) = i$. On the other hand, since $e$ is a bad edge, we have $\ind(k_{\min}) \le i-2$. Since $\delta \le (\gamma-1) k_{\min}$, by Lemma~\ref{lem:change}, $\ind(k_{f_{\min}})$ is at most increased by $1$, which menas $\ind(k_{f_{\min}}) \le i-1$ after the weight change. Again by Lemma~\ref{lem:change}, for any edge $f$ such that $k_f$ increases, $\ind(k_f) \le \ind(k_{f_{\min}}) \le i-1$. This concludes the first part of the claim.

    Now we prove the second part of the claim. Since $\ind(k_{\max})-\ind(k_{\min}) \ge 2$, $\delta \le (\gamma-1) k_{\min} \le \frac{\gamma-1}{\gamma} k_{\max}$. By Lemma~\ref{lem:change}, $\ind(k_{f_{\max}})$ at most decrease by $1$, which means $\ind(k_{f_{\max}}) \ge i-1$. Again by Lemma~\ref{lem:change}, for any edge $f$ such that $k_f$ decrease, $\ind(k_f) \ge \ind(k_{f_{\max}}) \ge i-1 \ge 2$ after the weight change. This concludes the second part of the claim.
\end{proof}

By Claim~\ref{cla:interval-contained}, we prove that the interval $I=[K_{\min},K_{\max}]$ (which was defined using the initial graph $G^{init}$) is the correct range of strengths to focus on. The algorithm gives a $\gamma^2$-balanced assignment if it terminates since there is no bad hyperedge. Therefore, to prove Theorem~\ref{thm:balance}, it is sufficient to prove that the running of ${\rm Balance}(w^{init},\ell)$ takes $m^{O(\log_{\gamma} m)}$ time.

\begin{claim} \label{cla:time}
    The running time of ${\rm Balance}(w^{init},\ell)$ is $m^{O(\log_{\gamma} m)}$.
\end{claim}

\begin{proof}
    Since calculating the strengths of the edges, updating the weights can both be done in polynomial time. To prove the lemma, it is sufficient to prove that the number of times of updating the weight function is $m^{O(\log_{\gamma} m)}$. Let $T_i$ be the upper bound of the number of times of updating the weight function during a call of ${\rm Balance}(w,i)$. We prove that $T_i \le (2mn^2+1)(T_{i-1}+1)$ for any $3 \le i \le \ell$.
    
    To prove the statement, it is sufficient to prove that the algorithm goes through the while loop at most $2mn^2$ times. Throughout out the run, let $S$ be the set of edges $f$ such that $\ind(k_f) = i$ and $f$ is in $F_e^+$ where $\ind(e) = i$. We maintain two potential functions $\phi_1$ and $\phi_2$ where $\phi_1 = \sum_{f \in S} w(f)$ and $\phi_2 = \card{S}$. In the beginning, $S \subseteq F$, so $\phi_1 \le \sum_{f \in F} w(f) = m$ and $\phi_2 \le \card{F} = m \cdot \binom{n}{2} < mn^2$. In each while loop, $f_{\max}$ is a member of $S$ and $\ind(f_{\min}) \le i-2$. By Claim~\ref{cla:interval-contained}, $S$ never gets new element and the weight of each edge $f$ such $\ind(f)=i$ never increases, which means both potential function is non-increasing. If $\delta = (\gamma-1) k_{\min}$, the weight of $k_{max}$ is decreased by at least $(\gamma-1)k_{\min}\geq k_{\min} \ge K_{\min} \ge \frac{1}{n^2}$. In this case, $\phi_1$ is decreased by at least $\frac{1}{n^2}$. If $\delta = w(f_{\max})$, then $f_{\max}$ becomes $0$ weights after the weight change, which means $f_{\max}$ is no longer a member of $S$. In this case, $\phi_2$ is decreased by $1$. So the total number of times the algorithm go through the while loop is at most $\frac{m}{\frac{1}{n^2}}+mn^2=2mn^2$.

    Now we have $T_i \le (2mn^2+1)(T_{i-1}+1)$, which means $T_i + 1 \le (2mn^2+1)(T_{i-1}+1)+1 \le (2mn^2+2)(T_{i-1}+1)$. Since $T_2 = 0$, we have $T_{\ell} \le (2mn^2+2)^{\ell-2}$, which means $T_{\ell} = m^{O(\log_{\gamma} m)}$ (here we used the assumption that $m \ge n$ and the fact that $\ell \le \log_{\gamma} (mn^2)$).
\end{proof}

By Claim~\ref{cla:interval-contained} and Claim~\ref{cla:time}, the algorithm correctly outputs a $\gamma^2$-balanced assignment in $m^{O(\log m)}$ time.


==> streaming.tex <==
There is a process (see Section 2.2 of~\cite{McGregor14}) that converts any graph sparsifier algorithm to an insertion only streaming algorithm. The argument also works for hypergraph sparsifiers.

\begin{lemma} [\cite{McGregor14}] \label{lem:streaming}
    Given an algorithm that finds a $(1\pm \eps)$-approximate cut sparsifier of a hypergraph of size at most $f(n, \eps, d)$ with probability at least $1-n^{-d}$, there exists an insertion only streaming algorithm to compute a $(1\pm\eps)$-approximate cut sparsifier of size $2\log(m/n) \cdot f(n,\frac{\eps}{2\log(m/n)})$ that stores at most $2\log^2(m/n)\cdot f(n,\frac{\eps}{2\log(m/n)})$ hyperedges at any given time with high probability.
\end{lemma}

\begin{corollary}
    For any $0<\eps<1$, there exists an randomized insertion only streaming algorithm that constructs $(1 \pm \eps)$-approximate cut sparsifier of $H$ of size $O(\frac{n\log n \log^3(m/n)}{\eps^2})$ with high probability and uses $O(\frac{n\log n \log^4(m/n)}{\eps^2})$ space.
\end{corollary}



